Predicting aqueous and electrochemical stability of 2D materials from extended Pourbaix analyses

A key challenge for computational discovery of electrocatalytic materials is the reliable prediction of thermodynamic stability in aqueous environment and under different electrochemical conditions. In this work, we first evaluate the electrochemical stability of more than 3000 two-dimensional (2D) materials using conventional Pourbaix diagrams (CPDs). Due to the complete neglect of thermodynamic barriers along the (often complex) reaction pathways, the vast majority of the materials are predicted to be unstable even though some are known to be stable in practice. We then introduce an analysis based on the surface Pourbaix diagram (SPD) including 'early intermediate states' that represent the first steps of the key surface passivation and dissolution reactions. The SPD framework is applied to the 2D materials MoS$_2$, phosphorene, and the MXene Ti$_2$C, all of which are predicted to be unstable by the CPD. For MoS$_2$, our approach reproduces the experimental pH-U stability window as well as the experimental desulphurization potential. For phosphorene and Ti2$_C$, the SPD approach is used to investigate the spontaneous degradation mechanism and the potential-dependent surface termination, respectively, again yielding good agreement with experiments. The SPD-based stability analysis emerges as a versatile and quantitative method for prediction of stability and investigation of surface structures in electrochemical environments.

==> table2.tex <==
 \begin{table}[]
\begin{tabular}{lc|cccccc}
\hline
\multirow{3}{*}{Formula} & \multirow{3}{*}{$\Delta H_{hull}$ (eV/atom)} & \multicolumn{6}{c}{$\Delta G_{pbx}$ (eV/atom)}                                 \\ \cline{3-8} 
                         &                                              & \multicolumn{3}{c|}{HER Conditions}      & \multicolumn{3}{c}{OER conditions} \\
                         &                                              & pH 0 & pH 7 & \multicolumn{1}{c|}{pH 14} & pH 0      & pH 7      & pH 14    \\ 
			\hline
\ce{CuTe} & 0.0 & -0.089 & -0.089 & \multicolumn{1}{l|}{-0.089} & 3.597 & 3.483 & 3.475 \\
\ce{FeO2} & 0.0 & 0.568 & 0.291 & \multicolumn{1}{l|}{0.268} & -0.098 & -0.256 & -0.249 \\
\ce{HfMo2O8} & 0.0 & -0.064 & -0.064 & \multicolumn{1}{l|}{-0.064} & -0.064 & -0.064 & -0.064 \\
\ce{HgSe} & 0.040 & -0.205 & -0.049 & \multicolumn{1}{l|}{0.159} & 2.574 & 2.583 & 2.575 \\
\ce{HgTe} & 0.044 & -0.159 & -0.159 & \multicolumn{1}{l|}{-0.159} & 3.265 & 3.273 & 3.266 \\
\ce{InHO4Se} & 0.0 & 0.189 & 0.232 & \multicolumn{1}{l|}{0.292} & -0.054 & -0.042 & 0.076 \\
\ce{KO3} & 0.0 & 1.559 & 1.454 & \multicolumn{1}{l|}{1.407} & 0.023 & -0.083 & -0.129 \\
\ce{MgH2O2} & 0.009 & 0.168 & 0.002 & \multicolumn{1}{l|}{-0.136} & 0.168 & 0.002 & -0.079 \\
\ce{MnO2} & 0.018 & 0.542 & 0.265 & \multicolumn{1}{l|}{0.142} & -0.277 & -0.386 & -0.385 \\
\ce{MnRe2O8} & 0.000 & 0.044 & -0.032 & \multicolumn{1}{l|}{-0.065} & -0.109 & -0.109 & -0.109 \\
\ce{Mo2Ta2O11} & 0.001 & -0.063 & -0.063 & \multicolumn{1}{l|}{-0.063} & -0.063 & -0.063 & -0.063 \\
\ce{Mo2ZrO8} & 0.011 & -0.059 & -0.059 & \multicolumn{1}{l|}{-0.059} & -0.059 & -0.059 & -0.059 \\
\ce{MoO3} & 0.0 & -0.022 & -0.022 & \multicolumn{1}{l|}{-0.022} & -0.636 & -0.565 & -0.358 \\
\ce{Na2GeH6O6} & 0.000 & 0.046 & -0.009 & \multicolumn{1}{l|}{-0.064} & 0.046 & 0.015 & 0.013 \\
\ce{NaBH4O4} & 0.014 & 0.018 & -0.023 & \multicolumn{1}{l|}{-0.064} & 0.018 & -0.005 & -0.006 \\
\ce{NaCHO3} & 0.0 & 0.052 & -0.017 & \multicolumn{1}{l|}{-0.068} & 0.052 & 0.013 & 0.011 \\
\ce{NaO3} & 0.0 & 1.566 & 1.462 & \multicolumn{1}{l|}{1.359} & 0.030 & -0.076 & -0.177 \\
\ce{NiHO2} & 0.0 & 0.427 & 0.219 & \multicolumn{1}{l|}{0.219} & 0.119 & -0.088 & -0.118 \\
\ce{NiO2} & 0.0 & 0.836 & 0.560 & \multicolumn{1}{l|}{0.56} & 0.017 & -0.260 & -0.299 \\
\ce{NiRe2O8} & 0.0 & 0.038 & -0.038 & \multicolumn{1}{l|}{-0.037} & -0.195 & -0.271 & -0.281 \\
\ce{O2Se} & 0.023 & 0.590 & 0.692 & \multicolumn{1}{l|}{0.832} & -0.187 & 0.053 & 0.327 \\
\ce{O3Sb2} & 0.0 & -0.072 & -0.071 & \multicolumn{1}{l|}{-0.072} & 0.657 & 0.658 & 0.657 \\
\ce{O4PSb} & 0.005 & -0.118 & -0.070 & \multicolumn{1}{l|}{0.082} & 0.285 & 0.285 & 0.365 \\
\ce{OsSe2} & 0.0 & -0.173 & 0.034 & \multicolumn{1}{l|}{0.312} & 4.532 & 4.602 & 5.142 \\
\ce{PbSrO8S2} & 0.025 & 0.120 & 0.050 & \multicolumn{1}{l|}{0.07} & -0.057 & -0.032 & 0.030 \\
\ce{PdO2} & 0.0 & 0.870 & 0.868 & \multicolumn{1}{l|}{0.87} & -0.265 & -0.266 & -0.265 \\
\ce{PdPt3O8} & 0.0 & 0.767 & 0.765 & \multicolumn{1}{l|}{0.766} & -0.075 & -0.075 & -0.075 \\
\ce{PdRe2O8} & 0.000 & 0.105 & 0.104 & \multicolumn{1}{l|}{0.104} & -0.215 & -0.215 & -0.215 \\
\ce{PdSe2} & 0.004 & -0.056 & 0.048 & \multicolumn{1}{l|}{0.211} & 2.523 & 2.561 & 2.969 \\
\ce{PtO2} & 0.006 & 0.720 & 0.719 & \multicolumn{1}{l|}{0.72} & -0.273 & -0.274 & -0.273 \\
\ce{PtSe2} & 0.0 & -0.207 & -0.083 & \multicolumn{1}{l|}{0.084} & 2.654 & 2.721 & 3.264 \\
\ce{Re2ZnO8} & 0.0 & -0.014 & -0.039 & \multicolumn{1}{l|}{-0.039} & -0.247 & -0.272 & -0.272 \\
\ce{ReSe2} & 0.0 & -0.146 & 0.063 & \multicolumn{1}{l|}{0.339} & 4.437 & 4.506 & 5.047 \\
\ce{Sb2Se3} & 0.0 & -0.065 & 0.123 & \multicolumn{1}{l|}{0.372} & 4.017 & 4.079 & 4.565 \\
\ce{SrH4O3} & 0.016 & 0.121 & 0.017 & \multicolumn{1}{l|}{-0.055} & 0.121 & 0.017 & -0.055 \\
\ce{V2O5} & 0.0 & -0.015 & -0.016 & \multicolumn{1}{l|}{-0.015} & -0.366 & -0.367 & -0.253 \\
\ce{VO5P} & 0.0 & -0.030 & -0.028 & \multicolumn{1}{l|}{0.103} & -0.069 & -0.028 & 0.103 \\
			\hline
		\end{tabular}
	\caption{An example table.}
	\label{table:example_table}
\end{table}

